ArborX: A Performance Portable Geometric Search Library

Searching for geometric objects that are close in space is a fundamental component of many applications. The performance of search algorithms comes to the forefront as the size of a problem increases both in terms of total object count as well as in the total number of search queries performed. Scientific applications requiring modern leadership-class supercomputers also pose an additional requirement of performance portability, i.e. being able to efficiently utilize a variety of hardware architectures. In this paper, we introduce a new open-source C++ search library, ArborX, which we have designed for modern supercomputing architectures. We examine scalable search algorithms with a focus on performance, including a highly efficient parallel bounding volume hierarchy implementation, and propose a flexible interface making it easy to integrate with existing applications. We demonstrate the performance portability of ArborX on multi-core CPUs and GPUs, and compare it to the state-of-the-art libraries such as Boost.Geometry.Index and nanoflann.

==> figures/bvh.tex <==
\begin{tikzpicture}[
    internal_node/.style={circle, draw=black, fill=none, text centered, anchor=north, text=black},
    black_node/.style={circle, draw=black, fill=black, text centered, anchor=north, text=black},
    red_node/.style={circle, draw=red, fill=red, text centered, anchor=north, text=black},
    blue_node/.style={circle, draw=blue, fill=blue, text centered, anchor=north, text=black},
    yellow_node/.style={circle, draw=yellow, fill=yellow, text centered, anchor=north, text=black},
  ]
  % Circles
  \filldraw[fill=black, draw=black] (-6, -2) circle (0.1);
  \filldraw[fill=red, draw=red] (-5, -1.8) circle (0.1);
  \filldraw[fill=blue, draw=blue] (-5.8, -1) circle (0.1);
  \filldraw[fill=yellow, draw=yellow] (-5.3, -1.5) circle (0.1);

  % Bounding boxes
  \draw[draw=black, text=black] (-6.6, -2.6) rectangle (-4.4, -0.4) node[pos=0.1] {0};
  \draw[draw=black, text=black] (-6.2, -2.2) rectangle (-5.6, -0.8) node[pos=0.5] {1};
  \draw[draw=black, text=black] (-5.5, -2.2) rectangle (-4.8, -0.8) node[pos=0.7]
  {2};

  % Tree
  \node (root)[internal_node] {0}  [->, line width=1pt, sibling distance=3cm]
  child{
      node (internal_node_1)[internal_node]{1} [sibling distance=1cm]
      child{
        node (black)[black_node]{}
      }
      child{
        node (blue)[blue_node]{}
      }
  }
  child{
      node (internal_node_2)[internal_node]{2} [sibling distance=1cm]
      child{
        node (red)[red_node]{}
      }
      child{
        node (yellow)[yellow_node]{}
      }
  }
  ;

\end{tikzpicture}


==> figures/bvh_overlapping.tex <==
\begin{tikzpicture}
  % First row
  \filldraw (-4, 0) rectangle (-2, 0.1);
  \filldraw (-1 ,0) rectangle (1, 0.1);
  \filldraw (2, 0) rectangle (4, 0.1);

  % Second row
  \filldraw (-2.5, -1) rectangle (-0.5, -0.9);
  \filldraw (0.5, -1) rectangle (2.5, -0.9);

  % Third row
  \filldraw (-4, -2) rectangle (-2, -1.9);
  \filldraw (-1, -2) rectangle (1, -1.9);
  \filldraw (2, -2) rectangle (4, -1.9);

  % Fourth row
  \filldraw (-2.5, -3) rectangle (-0.5, -2.9);
  \filldraw (0.5, -3) rectangle (2.5, -2.9);

  %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
  % First set of bounding boxes %
  %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
  % First bounding box
  \draw[draw=blue, line width=1.5pt] (-4.1, -0.1) rectangle (4.1, 0.2);

  % Second bounding box
  \draw[draw=blue, line width=1.5pt] (-2.6, -1.1) rectangle (2.6, -0.8);

  % Third bounding box
  \draw[draw=blue, line width=1.5pt] (-4.1, -2.1) rectangle (4.1, -1.8);

  % Fourth bounding box
  \draw[draw=blue, line width=1.5pt] (-2.6, -3.1) rectangle (2.6, -2.8);

  %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
  % Second set of bounding boxes %
  %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

  % First bounding box
  \draw[draw=green, line width=1.5pt] (-4.2, -2.2) rectangle (-1.8, 0.3);

  % Second bounding box
  \draw[draw=green, line width=1.5pt] (-2.7, -3.2) rectangle (-0.3, -0.7);

  % Third bounding box
  \draw[draw=green, line width=1.5pt] (-1.2, -2.2) rectangle (1.2, 0.3);

  % Fourth bounding box
  \draw[draw=green, line width=1.5pt] (0.4, -3.2) rectangle (2.7, -0.7);

  % Fifth bounding box
  \draw[draw=green, line width=1.5pt] (1.8, -2.2) rectangle (4.2, 0.3);

  % Query
  \filldraw[fill=red, draw=red] (-0.05, -2.5) rectangle (0.05, 0.5);
\end{tikzpicture}


==> figures/bvh_range_division.tex <==
\begin{tikzpicture}[
    box/.style={rectangle, draw=none, fill=Tblue, text=Tblue, text centered, anchor=north},
    v_box/.style={rectangle, draw=none, fill=Torange, text=black, align=center, anchor=north, font=\bf},
    internal_parent/.style={circle, draw=none, fill=yellow, text centered, anchor=north, text=black, font=\bf},
    internal_node/.style={circle, draw=none, fill=Tgreen, text centered, anchor=north, text=black, font=\bf},
    leaf_node/.style={circle, draw=none, fill=Tred, text centered, anchor=north, text=black, font=\bf},
    level distance=0.5cm,
    growth parent anchor=south
  ]
  %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
  \node (internal_node_0)[internal_node,
  ]{0}
    ;
  {[on background layer]
  \node (box_0)[box, right=-0.5cm of internal_node_0]{
    000000000000000000000000000000000000000000000000000000000000000000000000}
    ;
    }
  %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
  \node (internal_parent_0)[internal_parent,
    right= 5.25cm of internal_node_0]{} [->, line width=1pt]
    child{
      node (internal_node_3)[internal_node]{3}
    }
    child{
      node (internal_node_4)[internal_node]{4}
    }
    ;
  {[on background layer]
  \node (box_3)[box,
  left= -0.5cm of internal_node_3]{
    00000000000000000000000000000000}
    ;
  \node (box_4)[box,
  right= -0.5cm of internal_node_4]{
    00000000000000000000000000000000}
    ;
    }
  %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
  \node (internal_parent_3)[internal_parent, left= 2cm of internal_node_3]{} [->, line width=1pt]
    child{
      node (internal_node_1)[internal_node]{1}
    }
    child{
      node (internal_node_2)[internal_node]{2}
    }
    ;
  \node (internal_parent_4)[internal_parent, right= 2cm of internal_node_4]{} [->, line width=1pt]
    child{
      node (internal_node_5)[internal_node]{5}
    }
    child{
      node (internal_node_6)[internal_node]{6}
    }
    ;
  {[on background layer]
  \node (box_1)[box,
  left= -0.5cm of internal_node_1]{
    000000000000}
    ;
  \node (box_2)[box,
  right= -0.5cm of internal_node_2]{
    000000000000}
    ;
  \node (box_5)[box,
  left= -0.5cm of internal_node_5]{
    000000000000}
    ;
  \node (box_6)[box,
  right= -0.5cm of internal_node_6]{
    000000000000}
    ;
    }
  %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
  \node (internal_parent_1)[internal_parent, left= 0.5cm of internal_node_1]{} [->, line width=1pt]
    child{
      node (leaf_node_0)[leaf_node]{0}[->, line width=1pt]
      child{
        node (v_box_0)[v_box]{0\\0\\0\\0\\1}
      }
    }
    child{
      node (leaf_node_1)[leaf_node]{1}[->, line width=1pt]
      child{
        node (v_box_1)[v_box]{0\\0\\0\\1\\0}
      }
    }
    ;
  \node (internal_parent_2)[internal_parent, right= 0.5cm of internal_node_2]{} [->, line width=1pt]
    child{
      node (leaf_node_2)[leaf_node]{2}[->, line width=1pt]
      child{
        node (v_box_2)[v_box]{0\\1\\0\\0\\0}
      }
    }
    child{
      node (leaf_node_3)[leaf_node]{3}[->, line width=1pt]
      child{
        node (v_box_3)[v_box]{0\\1\\1\\0\\0}
      }
    }
    ;
  \node (internal_parent_5)[internal_parent, left= 0.5cm of internal_node_5]{} [->, line width=1pt]
    child{
      node (leaf_node_4)[leaf_node]{4}[->, line width=1pt]
      child{
        node (v_box_4)[v_box]{1\\0\\0\\0\\0}
      }
    }
    child{
      node (leaf_node_5)[leaf_node]{5}[->, line width=1pt]
      child{
        node (v_box_5)[v_box]{1\\0\\0\\0\\1}
      }
    }
    ;
  \node (internal_parent_6)[internal_parent, right= 0.5cm of internal_node_6]{} [->, line width=1pt]
    child{
      node (leaf_node_6)[leaf_node]{6}[->, line width=1pt]
      child{
        node (v_box_6)[v_box]{1\\1\\0\\0\\0}
      }
    }
    child{
      node (leaf_node_7)[leaf_node]{7}[->, line width=1pt]
      child{
        node (v_box_7)[v_box]{1\\1\\0\\0\\1}
      }
    }
    ;
\end{tikzpicture}

